Range Queries for Permutation Pattern Matching: Separations, Equivalences, and Applications

The problem of Permutation Pattern Matching (PPM) asks, given a permutation $\pi:[n]\to[n]$, viewed as the point set $P=\{(i,\pi(i)):i\in[n]\}$, and a pattern $\sigma$ of small length $k$, whether $P$ contains an order-isomorphic copy of $\sigma$. The PPM problem and its (exact and approximate) counting variants have been studied extensively in the literature. We consider a preprocessing-query version: after preprocessing $P$, one must determine whether a query $P'\subseteq P$ contains $\sigma$, where $P'$ is obtained by intersecting $P$ with a geometric shape (e.g., an axis-aligned rectangle or $k$ such rectangles). This naturally generalizes the classical range query problem in computational geometry, which corresponds to the case $|\sigma|=1$. We extend the study of this problem from patterns of length $2$ to patterns of length $3$ (and in some cases beyond), and prove new fine-grained equivalences, separations, and applications: (1) Single rectangle: For all patterns of length $3$, detection can be done with $\tilde{O}(n)$ preprocessing and $\tilde{O}(1)$ query time. The proof goes through a new tool of independent interest: reductions from rectangle queries to a simpler family of slab queries. (2) Multiple rectangles: For $\sigma=132$, detection is equivalent to the online set disjointness problem; we also show connections to online $k$-set disjointness. To our knowledge, this is the first equivalence between a PPM-type problem and online set disjointness, a problem playing a fundamental role in fine-grained complexity. (3) Counting: As applications, we obtain an $O(n^{1.725})$ time algorithm for exact counting of $5$-patterns based on the rectangle-to-slab reduction, improving upon [Beniamini and Lavee, ICALP 2025], and an $\tilde{O}(n^{7/4})$ approximate counting algorithm for $6$-patterns, the first to break the $O(n^2)$ barrier for $6$-patterns.

==> defs.tex <==
\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
\makeatletter
\let\oldabs\abs
\def\abs{\@ifstar{\oldabs}{\oldabs*}}
\makeatother

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{fact}{Fact}
\newtheorem{problem}{Problem}
\makeatletter
\renewcommand{\theproblem}{\arabic{problem}}
\@removefromreset{problem}{section}
\makeatother

\makeatletter
\renewenvironment{proof}[1][\proofname]{\par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item\relax
    {\bfseries\boldmath
        #1\@addpunct{.}}\hspace\labelsep\ignorespaces
}{%
    \popQED\endtrivlist\@endpefalse
}
\makeatother

\crefname{claim}{claim}{claims}
\Crefname{claim}{Claim}{Claims}

% Grid / canonical rectangles
\newcommand{\CR}[1]{\mathcal{C}(#1)}
\newcommand{\Grid}{\wpa{Grid}}
\newcommand{\slab}{S}

\newcommand{\alledges}{\textsc{AllEdgeInTriangle}\xspace}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\TT}{\mathcal{T}}

% Range-tree notation
\newcommand{\ver}{x}
\newcommand{\hor}{y}
\newcommand{\Tv}{T_{\ver}}
\newcommand{\Th}{T_{\hor}}

% Named subroutines / data structures
\newcommand{\AB}{\normalfont{\textsc{Query}_{12}}\xspace}
\newcommand{\intQuery}{{\normalfont{\textsc{132-SlabQuery}}}\xspace}
\newcommand{\shrink}{\normalfont{\textsc{Shrink}}\xspace}
\newcommand{\rank}{{\normalfont\textsc{Rank}}\xspace}

\newcommand{\brak}[1]{\left(#1\right)}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\sset}[1]{\{#1\}}
\newcommand{\poly}{\operatorname{poly}}

\newcommand{\mo}{O}
\newcommand{\TO}[1]{\tilde{\mo}(#1)}
\newcommand{\tf}{\tilde{O}}
\newcommand{\To}{\tilde{\mo}}

\newcommand{\eps}{\varepsilon}
\newcommand{\AC}{\mathcal{A}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\RR}{\mathcal{R}}

\makeatletter
\newcommand{\whp}{%
  w.h.p.\@ifnextchar.{\@gobble}{\xspace}%
}
\makeatother

\newcommand{\nemp}{\neq\emptyset}

\newcommand*{\ind}{\text{\usefont{U}{bbold}{m}{n}1}}
\newcommand{\indd}{\ind_{132}}
\newcommand{\inds}{\ind_{\sigma}}

\newcommand{\pppm}{{\normalfont\textsc{PartitionedPPM}}\xspace}
\newcommand{\cppm}{{\normalfont\textsc{ColorfulPPM}}\xspace}
\newcommand{\rppm}{{\normalfont\textsc{RectPPM}}\xspace}
\newcommand{\sppm}{{\normalfont\textsc{SlabPPM}}\xspace}
\newcommand{\rppmc}{{\normalfont\textsc{132-RectPPM}}\xspace}
\newcommand{\sppmc}{{\normalfont\textsc{132-SlabPPM}}\xspace}
\newcommand{\srppm}{{\normalfont\textsc{SingleRectPPM}}\xspace}

\newcommand{\si}{{\sigma^{-1}}}
\renewcommand{\phi}{\varphi}

\newcommand{\wpa}[1]{{\normalfont\textsc{#1}}\xspace}
\newcommand{\prba}{{\normalfont\textsc{OnlineSetDisj}}\xspace}
\newcommand{\prbb}{{\normalfont\textsc{$k$-OnlineSetDisj}}\xspace}
\newcommand{\prbd}{{\normalfont\textsc{OnlineSuccinctSetDisj}}\xspace}

